Entanglement Maximization and Mirror Symmetry in Two-Higgs-Doublet Models

We consider 2-to-2 scatterings of Higgs bosons in a CP-conserving two-Higgs-doublet model (2HDM) and study the implication of maximizing the entanglement in the flavor space, where the two doublets $\Phi_a$, $a=1,2$, can be viewed as a qubit: $\Phi_1=|0\rangle$ and $\Phi_2=|1\rangle$. More specifically, we compute the scattering amplitudes for $\Phi_a \Phi_b \to \Phi_c \Phi_d$ and require the outgoing flavor entanglement to be maximal for a full product basis such as the computational basis, which consists of $\{|00\rangle,|01\rangle,|10\rangle,|11\rangle\}$. In the unbroken phase and turning off the gauge interactions, entanglement maximization results in the appearance of an $U(2)\times U(2)$ global symmetry among the quartic couplings, which in general is broken softly by the mass terms. Interestingly, once the Higgs bosons acquire vacuum expectation values, maximal entanglement enforces an exact $U(2) \times U(2)$ symmetry, which is spontaneously broken to $U(1)\times U(1)$. As a byproduct, this gives rise to Higgs alignment as well as to the existence of 6 massless Nambu-Goldstone bosons. The $U(2)\times U(2)$ symmetry can be gauged to lift the massless Goldstones, while maintaining maximal entanglement demands the presence of a discrete $\mathrm{Z}_2$ symmetry interchanging the two gauge sectors. The model is custodially invariant in the scalar sector, and the inclusion of fermions requires a mirror dark sector, related to the standard one by the $\mathrm{Z}_2$ symmetry.

==> concurrence_GC/cccc.tex <==
\subsection{$\Phi^+\Phi^- \to \Phi^+\Phi^-$}

Results.
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures_GC/cccc.pdf}
    \caption{Matrix elements for the different channels of $\Phi^+\Phi^- \to \Phi^+\Phi^-$ scattering.}
    \label{fig::cccc}
\end{figure}


\begin{align}
    &\text{4-point} \; : \;
   \begin{bmatrix}
    2 {Z_1} & 0 & 0 & {Z_3}+{Z_4} \\
    0 & 2 {Z_5} & {Z_3}+{Z_4} & 0 \\
    0 & {Z_3}+{Z_4} & 2 {Z_5} & 0 \\
    {Z_3}+{Z_4} & 0 & 0 & 2 {Z_2} \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{1e}}^0 \; : \;
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & -\frac{{Z_1} {Z_3}}{2} \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    -\frac{{Z_1} {Z_3}}{2} & 0 & 0 & -\frac{{Z_3}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{1o}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{2e}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & -\frac{1}{8} ({Z_5}+{Z_4})^2 & -\frac{1}{8} ({Z_5}+{Z_4})^2 & 0 \\
    0 & -\frac{1}{8} ({Z_5}+{Z_4})^2 & -\frac{1}{8} ({Z_5}+{Z_4})^2 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{2o}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & -\frac{1}{8} ({Z_5}-{Z_4})^2 & \frac{1}{8} ({Z_5}-{Z_4})^2 & 0 \\
    0 & \frac{1}{8} ({Z_5}-{Z_4})^2 & -\frac{1}{8} ({Z_5}-{Z_4})^2 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{t_{1e}}^0 \; : \;
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & 0 \\
    0 & -\frac{{Z_1} {Z_3}}{2} & 0 & 0 \\
    0 & 0 & -\frac{{Z_1} {Z_3}}{2} & 0 \\
    0 & 0 & 0 & -\frac{{Z_3}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{t_{1o}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{t_{2e}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{1}{8} ({Z_5}+{Z_4})^2 \\
    0 & 0 & -\frac{1}{8} ({Z_5}+{Z_4})^2 & 0 \\
    0 & -\frac{1}{8} ({Z_5}+{Z_4})^2 & 0 & 0 \\
    -\frac{1}{8} ({Z_5}+{Z_4})^2 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{t_{2o}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{1}{8} ({Z_5}-{Z_4})^2 \\
    0 & 0 & \frac{1}{8} ({Z_5}-{Z_4})^2 & 0 \\
    0 & \frac{1}{8} ({Z_5}-{Z_4})^2 & 0 & 0 \\
    -\frac{1}{8} ({Z_5}-{Z_4})^2 & 0 & 0 & 0 \\
   \end{bmatrix}
   \end{align}



\begin{table}[h!]
\centering
    \begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\
        \hline
        \hline
            $\text{4-point} $ & $ \frac{4 {Z_1} | {Z_3}+{Z_4}| }{4 {Z_1}^2+({Z_3}+{Z_4})^2} $ & $ \frac{4 | {Z_5} ({Z_3}+{Z_4})| }{4 {Z_5}^2+({Z_3}+{Z_4})^2} $ & $ \frac{4 | {Z_5} ({Z_3}+{Z_4})| }{4 {Z_5}^2+({Z_3}+{Z_4})^2} $ & $ \frac{4 {Z_2} |
      {Z_3}+{Z_4}| }{4 {Z_2}^2+({Z_3}+{Z_4})^2} $ \\ \hline $
      P_{s_{1e}}^0 $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ & $ 0 $ & $ 0 $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ \\ \hline $
      P_{s_{1o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
      P_{s_{2e}}^0 $ & $ 0 $ & $ 1 $ & $ 1 $ & $ 0 $ \\ \hline $
      P_{s_{2o}}^0 $ & $ 0 $ & $ 1 $ & $ 1 $ & $ 0 $ \\ \hline $
      P_{t_{1e}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
      P_{t_{1o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
      P_{t_{2e}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
      P_{t_{2o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline 
\end{tblr}
\caption{Concurrence for each matrix element (row) over the computational basis (column).}
\label{tab::cccc1}
\end{table}


\begin{table}[h!]
\centering
\begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\   
        \hline
        \hline
$\text{4-point}$ & $ \frac{4 {Z_1} | {Z_3}+{Z_4}| }{4 {Z_1}^2+({Z_3}+{Z_4})^2} $ & $ \frac{4 | {Z_5} ({Z_3}+{Z_4})| }{4 {Z_5}^2+({Z_3}+{Z_4})^2} $ & $ \frac{4 | {Z_5} ({Z_3}+{Z_4})| }{4 {Z_5}^2+({Z_3}+{Z_4})^2} $ & $ \frac{4 {Z_2} |
      {Z_3}+{Z_4}| }{4 {Z_2}^2+({Z_3}+{Z_4})^2} $ \\ \hline $
    {s} $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ & $ \frac{4 \left({Z_5}^2+{Z_4}^2\right) | {Z_5} {Z_4}| }{{Z_5}^4+6 {Z_5}^2 {Z_4}^2+{Z_4}^4} $ & $ \frac{4 \left({Z_5}^2+{Z_4}^2\right) | {Z_5} {Z_4}| }{{Z_5}^4+6
      {Z_5}^2 {Z_4}^2+{Z_4}^4} $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ \\ \hline $
    {t} $ & $ \frac{4 {Z_1}^2 \left({Z_5}^2+{Z_4}^2\right)}{\left({Z_5}^2+{Z_4}^2\right)^2+4 {Z_1}^4} $ & $ \frac{2 | {Z_5} {Z_1} {Z_3} {Z_4}| }{| {Z_5} {Z_4}| ^2+| {Z_1} {Z_3}| ^2} $ & $ \frac{2 | {Z_5} {Z_1} {Z_3} {Z_4}| }{|
      {Z_5} {Z_4}| ^2+| {Z_1} {Z_3}| ^2} $ & $ \frac{4 {Z_3}^2 \left({Z_5}^2+{Z_4}^2\right)}{\left({Z_5}^2+{Z_4}^2\right)^2+4 {Z_3}^4} $ \\ \hline
\end{tblr}
\caption{Concurrence for each channel (row) over the computational basis (column), assuming degenerate masses for the respective propagators.}
\label{tab::cccc2}
\end{table}


==> concurrence_GC/cncn.tex <==
\subsection{$\Phi^+\Phi^0 \to \Phi^+\Phi^0$}

Matrix elements.
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures_GC/cncn.pdf}
    \caption{Matrix elements for the different channels of $\Phi^+\Phi^0 \to \Phi^+\Phi^0$ scattering.}
    \label{fig::cncn}
\end{figure}


\newgeometry{left=.5cm}
\begin{align}
    &\text{4-point} \; : \;
   \begin{bmatrix}
    {Z_1} & 0 & 0 & {Z_5} \\
    0 & {Z_3} & {Z_4} & 0 \\
    0 & {Z_4} & {Z_3} & 0 \\
    {Z_5} & 0 & 0 & {Z_2} \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_1}^\pm \; : \;
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & -\frac{{Z_5} {Z_1}}{2} \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    -\frac{{Z_5} {Z_1}}{2} & 0 & 0 & -\frac{{Z_5}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{s_2}^\pm \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & -\frac{{Z_4}^2}{2} & -\frac{{Z_3} {Z_4}}{2} & 0 \\
    0 & -\frac{{Z_3} {Z_4}}{2} & -\frac{{Z_3}^2}{2} & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{u_1}^\pm \; : \;
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & 0 \\
    0 & 0 & -\frac{{Z_1} {Z_4}}{2} & 0 \\
    0 & -\frac{{Z_1} {Z_4}}{2} & 0 & 0 \\
    0 & 0 & 0 & -\frac{{Z_4}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{u_2}^\pm \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{{Z_5} {Z_3}}{2} \\
    0 & -\frac{{Z_5}^2}{2} & 0 & 0 \\
    0 & 0 & -\frac{{Z_3}^2}{2} & 0 \\
    -\frac{{Z_5} {Z_3}}{2} & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{1e}}^0 \; : \;
   \begin{bmatrix}
    -{Z_1}^2 & 0 & 0 & 0 \\
    0 & -\frac{1}{2} {Z_1} ({Z_3}+{Z_4}) & 0 & 0 \\
    0 & 0 & -{Z_1} {Z_3} & 0 \\
    0 & 0 & 0 & -\frac{1}{2} {Z_3} ({Z_3}+{Z_4}) \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{1o}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{2e}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) \\
    0 & 0 & -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) & 0 \\
    0 & -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) & 0 & 0 \\
    -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{2o}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & \frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) \\
    0 & 0 & -\frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) & 0 \\
    0 & -\frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) & 0 & 0 \\
    \frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) & 0 & 0 & 0 \\
   \end{bmatrix}
   \end{align}

\restoregeometry

\begin{table}[h!]
\centering
    \begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\
        \hline
        \hline
        4-point &  $ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $ & $ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $ & $ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $ & $ \frac{2 {Z_2} | {Z_5}| }{{Z_5}^2+{Z_2}^2} $ \\
        \hline
        {$P_{s_1}^\pm$} &$ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $&$ 0 $&$ 0 $&$ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2}$ \\
        \hline
        {$P_{s_2}^\pm$} &$ 0 $&$ \frac{2 | {Z_3}|  | {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ \frac{2 | {Z_3}|  | {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ 0 $\\
        \hline
        {$P_{u_1}^\pm$} &$ 0 $&$ 0 $&$ 0 $&$ 0 $\\
        \hline
        {$P_{u_2}^\pm$} &$ 0 $&$ 0 $&$ 0 $&$ 0 $\\
        \hline
        {$P_{t_{1e}}^0$} &$ 0 $&$ 0 $&$ 0 $&$ 0$ \\
        \hline
        {$P_{t_{1o}}^0$} &$ 0 $&$ 0 $&$ 0 $&$ 0$ \\
        \hline
        {$P_{t_{2e}}^0$} &$ 0 $&$ 0 $&$ 0 $&$ 0$ \\
        \hline
        {$P_{t_{2o}}^0$} &$ 0 $&$ 0 $&$ 0 $&$ 0$ \\
        \hline
\end{tblr}
\caption{Concurrence for each matrix element (row) over the computational basis (column).}
\label{tab::cncn1}
\end{table}


\newgeometry{left=1cm}
\begin{table}[h!]
\begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\   
        \hline
        \hline
        $\text{4-point}$ &$ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $&$ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ \frac{2 {Z_2} | {Z_5}| }{{Z_5}^2+{Z_2}^2} $ \\ \hline 
        ${s}$ &$ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $&$ \frac{2 | {Z_3}|  | {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ \frac{2 | {Z_3}|  | {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $ \\  \hline
        ${u}$ &$ \frac{2 \left| {Z_5} {Z_1}^2 {Z_3}\right| }{| {Z_5} {Z_3}| ^2+{Z_1}^4} $&$ \frac{2 {Z_5}^2 {Z_1} | {Z_4}| }{| {Z_1} {Z_4}| ^2+{Z_5}^4} $&$ \frac{2 {Z_1} {Z_3}^2 | {Z_4}| }{| {Z_1} {Z_4}| ^2+{Z_3}^4} $&$ \frac{2
          \left| {Z_5} {Z_3} {Z_4}^2\right| }{| {Z_5} {Z_3}| ^2+{Z_4}^4} $ \\ \hline
        ${t}$ &$ \frac{8 {Z_1}^2 | {Z_5} ({Z_3}+3 {Z_4})| }{{Z_5}^2 ({Z_3}+3 {Z_4})^2+16 {Z_1}^4} $&$ \frac{4 \left| {Z_1} ({Z_3}+{Z_4}) \left(2 {Z_5}^2+{Z_4} ({Z_3}+{Z_4})\right)\right| }{\left(2 {Z_5}^2+{Z_4}
          ({Z_3}+{Z_4})\right)^2+4 {Z_1}^2 ({Z_3}+{Z_4})^2} $&$ \frac{8 \left| {Z_1} {Z_3} \left(2 {Z_5}^2+{Z_4} ({Z_3}+{Z_4})\right)\right| }{\left(2 {Z_5}^2+{Z_4} ({Z_3}+{Z_4})\right)^2+16 {Z_1}^2 {Z_3}^2} $&$ \frac{| {Z_5} {Z_3}
          ({Z_3}+{Z_4}) ({Z_3}+3 {Z_4})| }{| {Z_3} ({Z_3}+{Z_4})| ^2+\frac{1}{4} {Z_5}^2 ({Z_3}+3 {Z_4})^2} $ \\ \hline
\end{tblr}
\caption{Concurrence for each channel (row) over the computational basis (column), assuming degenerate masses for the respective propagators.}
\label{tab::cncn2}
\end{table}

\restoregeometry

==> concurrence_GC/nncc.tex <==
\subsection{${\Phi^0}^\dag\Phi^0 \to \Phi^+\Phi^-$}

Matrix elements.
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures_GC/nncc.pdf}
    \caption{Matrix elements for the different channels of ${\Phi^0}^\dag\Phi^0 \to \Phi^+\Phi^-$ scattering.}
    \label{fig::nncc}
\end{figure}


\begin{align}
    & \text{4-point} \; : \;
   \begin{bmatrix}
    {Z_1} & 0 & 0 & {Z_3} \\
    0 & {Z_4} & {Z_5} & 0 \\
    0 & {Z_5} & {Z_4} & 0 \\
    {Z_3} & 0 & 0 & {Z_2} \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{1e}}^0 \; : \;   \begin{bmatrix}
    -{Z_1}^2 & 0 & 0 & -{Z_1} {Z_3} \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    -\frac{1}{2} {Z_1} ({Z_3}+{Z_4}) & 0 & 0 & -\frac{1}{2} {Z_3} ({Z_3}+{Z_4}) \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{1o}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{2e}}^0 \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) & -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) & 0 \\
    0 & -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) & -\frac{1}{8} ({Z_5}+{Z_4}) (2 {Z_5}+{Z_3}+{Z_4}) & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{s_{2o}}^0 \; : \;   
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & \frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) & -\frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) & 0 \\
    0 & -\frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) & \frac{1}{8} ({Z_5}-{Z_4}) (2 {Z_5}-{Z_3}-{Z_4}) & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{u_{1}}^\pm \; : \;
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & 0 \\
    0 & 0 & -\frac{{Z_1} {Z_4}}{2} & 0 \\
    0 & -\frac{{Z_1} {Z_4}}{2} & 0 & 0 \\
    0 & 0 & 0 & -\frac{{Z_4}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{u_{2}}^\pm \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{{Z_3}^2}{2} \\
    0 & -\frac{{Z_5} {Z_3}}{2} & 0 & 0 \\
    0 & 0 & -\frac{{Z_5} {Z_3}}{2} & 0 \\
    -\frac{{Z_5}^2}{2} & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{t_{1}}^\pm \; : \;
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & 0 \\
    0 & -\frac{{Z_5} {Z_1}}{2} & 0 & 0 \\
    0 & 0 & -\frac{{Z_5} {Z_1}}{2} & 0 \\
    0 & 0 & 0 & -\frac{{Z_5}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
   &\nonumber P_{t_{2}}^\pm \; : \;
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{{Z_3}^2}{2} \\
    0 & 0 & -\frac{{Z_3} {Z_4}}{2} & 0 \\
    0 & -\frac{{Z_3} {Z_4}}{2} & 0 & 0 \\
    -\frac{{Z_4}^2}{2} & 0 & 0 & 0 \\
   \end{bmatrix}
   \end{align}


\begin{table}[h!]
\centering
    \begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\
        \hline
        \hline
    $\text{4-point} $ & $ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $ & $ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $ & $ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $ & $ \frac{2 {Z_2} | {Z_5}| }{{Z_5}^2+{Z_2}^2} $ \\ \hline $
    P_{s_{1e}}^0 $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ & $ 0 $ & $ 0 $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ \\ \hline $
    P_{s_{1o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
    P_{s_{2e}}^0 $ & $ 0 $ & $ 1 $ & $ 1 $ & $ 0 $ \\ \hline $
    P_{s_{2o}}^0 $ & $ 0 $ & $ 1 $ & $ 1 $ & $ 0 $ \\ \hline $
    P_{u_{1}}^\pm $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
    P_{u_{2}}^\pm $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
    P_{t_{1}}^\pm $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
    P_{t_{2}}^\pm $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline
\end{tblr}
\caption{Concurrence for each matrix element (row) over the computational basis (column).}
\label{tab::nncc1}
\end{table}


\begin{table}[h!]
\centering
\begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\   
        \hline
        \hline
    $\text{4-point} $ & $ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $&$ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ \frac{2 | {Z_3} {Z_4}| }{{Z_3}^2+{Z_4}^2} $&$ \frac{2 {Z_2} | {Z_5}| }{{Z_5}^2+{Z_2}^2}$ \\ \hline $
    {s} $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ & $ \frac{2 \left| {Z_5} ({Z_3}+3 {Z_4}) \left(2 {Z_5}^2+{Z_4} ({Z_3}+{Z_4})\right)\right| }{{Z_5}^2 ({Z_3}+3 {Z_4})^2+\left(2 {Z_5}^2+{Z_4} ({Z_3}+{Z_4})\right)^2} $ & $
      \frac{2 \left| {Z_5} ({Z_3}+3 {Z_4}) \left(2 {Z_5}^2+{Z_4} ({Z_3}+{Z_4})\right)\right| }{{Z_5}^2 ({Z_3}+3 {Z_4})^2+\left(2 {Z_5}^2+{Z_4} ({Z_3}+{Z_4})\right)^2} $ & $ \frac{2 {Z_1} | {Z_3}| }{{Z_1}^2+{Z_3}^2} $ \\ \hline $
    {u} $ & $ \frac{2 {Z_1}^2 {Z_3}^2}{{Z_1}^4+{Z_3}^4} $ & $ \frac{2 | {Z_5} {Z_1} {Z_3} {Z_4}| }{| {Z_5} {Z_3}| ^2+| {Z_1} {Z_4}| ^2} $ & $ \frac{2 | {Z_5} {Z_1} {Z_3} {Z_4}| }{| {Z_5} {Z_3}| ^2+| {Z_1} {Z_4}| ^2} $ & $
      \frac{2 {Z_5}^2 {Z_4}^2}{{Z_5}^4+{Z_4}^4} $ \\ \hline $
    {t} $ & $ \frac{2 {Z_1}^2 {Z_3}^2}{{Z_1}^4+{Z_3}^4} $ & $ \frac{2 | {Z_5} {Z_1} {Z_3} {Z_4}| }{| {Z_5} {Z_1}| ^2+| {Z_3} {Z_4}| ^2} $ & $ \frac{2 | {Z_5} {Z_1} {Z_3} {Z_4}| }{| {Z_5} {Z_1}| ^2+| {Z_3} {Z_4}| ^2} $ & $
      \frac{2 {Z_5}^2 {Z_4}^2}{{Z_5}^4+{Z_4}^4} $ \\ \hline
\end{tblr}
\caption{Concurrence for each channel (row) over the computational basis (column), assuming degenerate masses for the respective propagators.}
\label{tab::nncc2}
\end{table}


==> concurrence_GC/nnnn.tex <==
\subsection{${\Phi^0}^\dag\Phi^0 \to {\Phi^0}^\dag\Phi^0$}

Matrix elements.
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures_GC/nnnn.pdf}
    \caption{Matrix elements for the different channels of ${\Phi^0}^\dag\Phi^0 \to {\Phi^0}^\dag\Phi^0$ scattering.}
    \label{fig::nnnn}
\end{figure}


\begin{align}
    &     \text{4-point} \; : \;
   \begin{bmatrix}
    2 {Z_1} & 0 & 0 & 2 {Z_5} \\
    0 & {Z_3}+{Z_4} & {Z_3}+{Z_4} & 0 \\
    0 & {Z_3}+{Z_4} & {Z_3}+{Z_4} & 0 \\
    2 {Z_5} & 0 & 0 & 2 {Z_2} \\
   \end{bmatrix} \\[1cm]
   &\nonumber P_{s_{1e}}^0 \; : \; 
   \begin{bmatrix}
    -2 {Z_1}^2 & 0 & 0 & -{Z_1} ({Z_3}+{Z_4}) \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    -{Z_1} ({Z_3}+{Z_4}) & 0 & 0 & -\frac{1}{2} ({Z_3}+{Z_4})^2 \\
   \end{bmatrix} \\[1cm]
   &\nonumber P_{s_{1o}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{s_{2e}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 & -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 & 0 \\
    0 & -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 & -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{s_{2o}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & -\frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 & \frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 & 0 \\
    0 & \frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 & -\frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{u_{1e}}^0 \; : \; 
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & 0 \\
    0 & 0 & -\frac{{Z_5} {Z_1}}{2} & 0 \\
    0 & -\frac{{Z_5} {Z_1}}{2} & 0 & 0 \\
    0 & 0 & 0 & -\frac{{Z_5}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{u_{1o}}^0 \; : \; 
   \begin{bmatrix}
    -\frac{{Z_1}^2}{2} & 0 & 0 & 0 \\
    0 & 0 & -\frac{{Z_5} {Z_1}}{2} & 0 \\
    0 & -\frac{{Z_5} {Z_1}}{2} & 0 & 0 \\
    0 & 0 & 0 & -\frac{{Z_5}^2}{2} \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{u_{2e}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{1}{8} ({Z_3}+{Z_4})^2 \\
    0 & -\frac{1}{8} ({Z_3}+{Z_4})^2 & 0 & 0 \\
    0 & 0 & -\frac{1}{8} ({Z_3}+{Z_4})^2 & 0 \\
    -\frac{1}{8} ({Z_3}+{Z_4})^2 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{u_{2o}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{1}{8} ({Z_3}+{Z_4})^2 \\
    0 & -\frac{1}{8} ({Z_3}+{Z_4})^2 & 0 & 0 \\
    0 & 0 & -\frac{1}{8} ({Z_3}+{Z_4})^2 & 0 \\
    -\frac{1}{8} ({Z_3}+{Z_4})^2 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{1e}}^0 \; : \; 
   \begin{bmatrix}
    -2 {Z_1}^2 & 0 & 0 & 0 \\
    0 & -{Z_1} ({Z_3}+{Z_4}) & 0 & 0 \\
    0 & 0 & -{Z_1} ({Z_3}+{Z_4}) & 0 \\
    0 & 0 & 0 & -\frac{1}{2} ({Z_3}+{Z_4})^2 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{1o}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{2e}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 \\
    0 & 0 & -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 & 0 \\
    0 & -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 & 0 & 0 \\
    -\frac{1}{8} (2 {Z_5}+{Z_3}+{Z_4})^2 & 0 & 0 & 0 \\
   \end{bmatrix}
    \\[1cm]
    &\nonumber P_{t_{2o}}^0 \; : \; 
   \begin{bmatrix}
    0 & 0 & 0 & -\frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 \\
    0 & 0 & \frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 & 0 \\
    0 & \frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 & 0 & 0 \\
    -\frac{1}{8} (-2 {Z_5}+{Z_3}+{Z_4})^2 & 0 & 0 & 0 \\
   \end{bmatrix}
   \end{align}

\begin{table}[h!]
\centering
    \begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\
        \hline
        \hline
$\text{4-point} $ & $ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $ & $ 1 $ & $ 1 $ & $ \frac{2 {Z_2} | {Z_5}| }{{Z_5}^2+{Z_2}^2} $ \\ \hline $
P_{s_{1e}}^0 $ & $ \frac{4 {Z_1} | {Z_3}+{Z_4}| }{4 {Z_1}^2+({Z_3}+{Z_4})^2} $ & $ 0 $ & $ 0 $ & $ \frac{4 {Z_1} | {Z_3}+{Z_4}| }{4 {Z_1}^2+({Z_3}+{Z_4})^2} $ \\ \hline $
P_{s_{1o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{s_{2e}}^0 $ & $ 0 $ & $ 1 $ & $ 1 $ & $ 0 $ \\ \hline $
P_{s_{2o}}^0 $ & $ 0 $ & $ 1 $ & $ 1 $ & $ 0 $ \\ \hline $
P_{u_{1e}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{u_{1o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{u_{2e}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{u_{2o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{t_{1e}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{t_{1o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{t_{2e}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline $
P_{t_{2o}}^0 $ & $ 0 $ & $ 0 $ & $ 0 $ & $ 0 $ \\ \hline
\end{tblr}
\caption{Concurrence for each matrix element (row) over the computational basis (column).}
\label{tab::nnnn1}
\end{table}



\newgeometry{left=1cm}
\begin{table}[h!]
\centering
\begin{tblr}{|c||c|c|c|c|}
        \hline
        Matrix & $(1,0,0,0)$ & $(0,1,0,0)$ & $(0,0,1,0)$ & $(0,0,0,1)$ \\   
        \hline
        \hline
$\text{4-point} $ & $ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $ & $ 1 $ & $ 1 $ & $ \frac{2 {Z_2} | {Z_5}| }{{Z_5}^2+{Z_2}^2} $ \\ \hline $
    {s} $ & $ \frac{4 {Z_1} | {Z_3}+{Z_4}| }{4 {Z_1}^2+({Z_3}+{Z_4})^2} $ & $ \frac{8 \left(4 {Z_5}^2+({Z_3}+{Z_4})^2\right) | {Z_5} ({Z_3}+{Z_4})| }{16 {Z_5}^4+24 {Z_5}^2 ({Z_3}+{Z_4})^2+({Z_3}+{Z_4})^4} $ & $ \frac{8 \left(4
      {Z_5}^2+({Z_3}+{Z_4})^2\right) | {Z_5} ({Z_3}+{Z_4})| }{16 {Z_5}^4+24 {Z_5}^2 ({Z_3}+{Z_4})^2+({Z_3}+{Z_4})^4} $ & $ \frac{4 {Z_1} | {Z_3}+{Z_4}| }{4 {Z_1}^2+({Z_3}+{Z_4})^2} $ \\ \hline $
    {u} $ & $ \frac{8 {Z_1}^2 ({Z_3}+{Z_4})^2}{16 {Z_1}^4+({Z_3}+{Z_4})^4} $ & $ \frac{8 {Z_1} | {Z_5}|  ({Z_3}+{Z_4})^2}{16 {Z_5}^2 {Z_1}^2+({Z_3}+{Z_4})^4} $ & $ \frac{8 {Z_1} | {Z_5}|  ({Z_3}+{Z_4})^2}{16 {Z_5}^2
      {Z_1}^2+({Z_3}+{Z_4})^4} $ & $ \frac{8 {Z_5}^2 ({Z_3}+{Z_4})^2}{16 {Z_5}^4+({Z_3}+{Z_4})^4} $ \\ \hline $
    {t} $ & $ \frac{{Z_1}^2 \left(4 {Z_5}^2+({Z_3}+{Z_4})^2\right)}{\frac{1}{16} \left(4 {Z_5}^2+({Z_3}+{Z_4})^2\right)^2+4 {Z_1}^4} $ & $ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $ & $ \frac{2 {Z_1} | {Z_5}| }{{Z_5}^2+{Z_1}^2} $ & $
      \frac{4 \left({Z_5}^2 ({Z_3}+{Z_4})^2+\frac{1}{4} ({Z_3}+{Z_4})^4\right)}{4 \left({Z_5}^2+\frac{1}{4} ({Z_3}+{Z_4})^2\right)^2+({Z_3}+{Z_4})^4} $ \\ \hline
\end{tblr}
\caption{Concurrence for each channel (row) over the computational basis (column), assuming degenerate masses for the respective propagators.}
\label{tab::nnnn2}
\end{table}

\restoregeometry

